No Rumours Please! A Multi-Indic-Lingual Approach for COVID Fake-Tweet Detection

The sudden widespread menace created by the present global pandemic COVID-19 has had an unprecedented effect on our lives. Man-kind is going through humongous fear and dependence on social media like never before. Fear inevitably leads to panic, speculations, and the spread of misinformation. Many governments have taken measures to curb the spread of such misinformation for public well being. Besides global measures, to have effective outreach, systems for demographically local languages have an important role to play in this effort. Towards this, we propose an approach to detect fake news about COVID-19 early on from social media, such as tweets, for multiple Indic-Languages besides English. In addition, we also create an annotated dataset of Hindi and Bengali tweet for fake news detection. We propose a BERT based model augmented with additional relevant features extracted from Twitter to identify fake tweets. To expand our approach to multiple Indic languages, we resort to mBERT based model which is fine-tuned over created dataset in Hindi and Bengali. We also propose a zero-shot learning approach to alleviate the data scarcity issue for such low resource languages. Through rigorous experiments, we show that our approach reaches around 89% F-Score in fake tweet detection which supercedes the state-of-the-art (SOTA) results. Moreover, we establish the first benchmark for two Indic-Languages, Hindi and Bengali. Using our annotated data, our model achieves about 79% F-Score in Hindi and 81% F-Score for Bengali Tweets. Our zero-shot model achieves about 81% F-Score in Hindi and 78% F-Score for Bengali Tweets without any annotated data, which clearly indicates the efficacy of our approach.

==> dataset_2.tex <==
\subsubsection{Monolingual Classifier}

For the Monolingual classifier we experimented with a variety of machine learning models on three main categories of datasets:

\begin{enumerate}
  \item Only Tweet Text Embeddings
  \item Tweet Text Embeddings + Tweet Features
  \item Tweet Text Embeddings + Tweet Features + User Features
\end{enumerate}

\usepackage{parskip}

For training models purely on tweet text embedding, we used BERT embedding with pre-trained weights.

%\begin{enumerate}

  %\item BERT\_CLS: Where we only used the output of vanilla BERT CLS token embeddings.
  
  %\item Sentence\_BERT\_NLI: Embeddings from sentence BERT model which is fine-tuned on NLI dataset. environment.
  
  %\item Sentence\_BERT\_NLI\_STSB: Embeddings from sentence BERT model which is fine-tuned on NLI and STSB dataset.
  
  %\item Sentence\_RoBERTa\_NLI: Embeddings from sentence RoBERTa model which is fine-tuned on NLI dataset.
  
  %\item Sentence\_RoBERTa\_NLI\_STSB: Embeddings from sentence RoBERTa model which is fine-tuned on NLI and STSB dataset.
  
%\end{enumerate}



We used 80\% of the Infodemic dataset for training and 20\% for testing. We trained an SVM classifier with kernel = ‘linear’, C=1, and gamma = 1 on all the above-mentioned text embeddings. Here, BERT\_CLS embeddings outperformed the other embedding models. This might be because of the fact that BERT\_CLS token is trained to perform well for classification tasks where as other models use the average of word embeddings to get the tweet text embeddings.



We trained the SVM with the same configuration for text embeddings + tweet features dataset, text embeddings + tweet features + user features dataset as well. We noticed the trend of decrease in accuracy on augmenting tweet and user features for SVM, maybe because our dataset was very small and the number of features were around 800. 



Since, BERT\_CLS embeddings outperformed all other embeddings, we trained Random Forest Classifier and Multi perceptron classifier as well. For the RFC used 400 estimators. For the MLP, we used 30 neurons in the first hidden layer and 10 neurons in the second hidden layer, with ReLU activation function for 10000 iterations. Here, our RFC model trained on text embeddings + tweet features + user features gave us 88\% Precision, 89\% Recall and 89\% F1-Score, which outperformed the current state-of-the-art on Infodemic dataset.

*******************

For mBERT Random Forest Classifier on combined English-hindi-bangla dataset we had 496 training samples and 123 test samples, which is again 80\% for train and 20\% for testing.


